Triple-entry Accounting, Blockchain and Next of Kin: Towards a Standardisation of Ledger Terminology

Triple-entry accounting (TEA) is simultaneously a novel application in the blockchain universe and one of the many concepts applied in blockchain technology. Its Wild Wild West status is accompanied by a lack of consistent and comprehensive set of categories, a state of play that impedes a proper apprehension of the technology, leading to contradictions and oversight of important nuances. To clearly delineate the confines of TEA within the world of blockchain, we provide building blocks to standardise its terminology. Particularly, we distinguish between essential elements such as accounting and bookkeeping, as well as between decentralised systems, distributed ledgers and distributed journals.

==> tables/assets.tex <==
\begin{table*}
\captionsetup{justification=centering}
\centering
\caption{\ac{DEFI} \ac{DAO} protocols and publicly traded companies universe examined.}
\scriptsize
\begin{tabular}{@{}rrrrcrrrcrrr@{}}\toprule
$\it{\ac{DEFI}}$ & \textbf{\acp{DEX}} && \textbf{\acp{PLF}} && \textbf{Yield aggregators} \\
\hphantom{$c$} & \acf{UNI}  && \acf{AAVE}  && \acf{YFI} \\
\hphantom{$c$} & \acf{CRV} && \acf{COMP} && \acf{IDLE} \\
\midrule
$\it{\ac{TradFi}}$ & \textbf{Exchanges} && \textbf{Banks} && \textbf{Asset managers} \\
\hphantom{$c$} & \acf{CBOE} && \acf{C} && \acf{BRK.B} \\
\hphantom{$c$} & \acf{NDAQ} && \acf{BAC} && \acf{MS} \\
\hphantom{$c$} & \acf{ICE} && \acf{WFC} &&  \acf{BLK} \\
\bottomrule
\end{tabular}
\label{tab:assets}
\end{table*}

==> tables/comparables.tex <==
\begin{tabular}{lrrrrr}
\toprule
{} & \multicolumn{2}{l}{Market Data} & Financial Data & \multicolumn{2}{l}{Estimations} \\
{} &        Prices &       Mkt Cap &            TVL &       Mkt Cap & Protocol Revenue \\
token &               &               &                &               &                  \\
\midrule
IDLE  &      2.037693 &  5.436950e+06 &   1.038275e+08 &  2.076550e+07 &     2.076550e+06 \\
COMP  &    200.170816 &  1.266899e+09 &   8.923174e+09 &  1.784635e+09 &     1.784635e+08 \\
UNI   &     17.058302 &  7.753293e+09 &   8.414520e+09 &  1.682904e+09 &     1.682904e+08 \\
BAL   &     17.534129 &  1.895901e+08 &   3.285260e+09 &  6.570519e+08 &     6.570519e+07 \\
AAVE  &    255.543328 &  3.459438e+09 &   1.434394e+10 &  2.868788e+09 &     2.868788e+08 \\
YFI   &  33025.884788 &  1.188961e+09 &   4.120927e+09 &  8.241853e+08 &     8.241853e+07 \\
\bottomrule
\end{tabular}


==> tables/dcf_cbanks.tex <==
\begin{table*}\centering

\caption{Banks' \ac{NPV} evaluation using \ac{DCF}.}
\label{table:cbanks_valuation}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule

\textbf{Citigroup}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  522,474.0 && 23,597.7 && 24,777.58 && 26,016.46 && 27,317.29 && 28,683.15 \\
Workforce expenses (\$M) & 	16,742.2 && 7,079.31 && 7,433.28 && 7,804.94 && 8,195.19 && 8,604.95\\
Net income (\$M) & 15,731.8 && 16,518.39 && 17,344.31 && 18,211.53 && 19,122.1 && 20,078.21\\
PV cashflows (\$M) & 15,731.8 && 15,006.1 && 14,313.88 && 13,653.59 && 13,023.76 && 12,422.99\\
PV terminal value (\$M) &  && && && && && 163,802.15\\
\textbf{Total PV (\$M)} & 247,954.28\\
\textbf{Total PV / C supply (\$)} & 128.02\\
\textbf{C market price (\$)} & 46.02 \\
\midrule

\textbf{Bank of America}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  31,394.0 && 32,963.7 && 34,611.88 && 36,342.48 && 38,159.6 && 40,067.58 \\
Workforce expenses (\$M) & 	9,418.2 && 9,889.11 && 10,383.56 && 10,902.74 && 11,447.88 && 12,020.28\\
Net income (\$M) & 21,975.8 && 23,074.59 && 24,228.32 && 25,439.74 && 26,711.72 && 28,047.31\\
PV cashflows (\$M) & 21,975.8 && 20,864.52 && 19,809.44 && 18,807.71 && 17,856.64 && 16,953.66\\
PV terminal value (\$M) &  && && && && && 211,690.06\\
\textbf{Total PV (\$M)} & 327,957.84\\
\textbf{Total PV / BAC supply (\$)} & 40.68\\
\textbf{BAC market price (\$)} & 31.15 \\
\midrule

\textbf{Well Fargo \& Co.}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  16,148.0 && 16,955.4 && 17,803.17 && 18,693.33 && 19,628.0 && 20,609.4 \\
Workforce expenses (\$M) & 	4,844.4 && 5,086.62 && 5,340.95 && 5,608.0 && 5,888.4 && 6,182.82\\
Net income (\$M) & 11,303.6 && 11,868.78 && 12,462.22 && 13,085.33 && 13,739.6 && 14,426.58 \\
PV cashflows (\$M) & 11,303.6 && 10,695.06 && 10,119.27 && 9,574.49 && 9,059.03 && 8,571.33\\
PV terminal value (\$M) &  && && && && && 102,944.03\\
\textbf{Total PV (\$M)} & 162,266.81\\
\textbf{Total PV / WFC supply (\$)} & 42.78\\
\textbf{WFC market price (\$)} & 39.17 \\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 30\% respectively. 
\end{table*}

==> tables/dcf_cex.tex <==
\begin{table*}\centering

\caption{\acp{CEX}' \ac{NPV} evaluation using \ac{DCF}.}
\label{table:cex_valuation}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule

\textbf{Intercontinental Exchange}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  5,882.0 && 6,176.1 && 6,484.9 && 6,809.15 && 7,149.61 && 7,507.09 \\
Workforce expenses (\$M) & 	1,764.6 && 1,852.83 && 1,945.47 && 2,042.74 && 2,144.88 && 2,252.13\\
Net income (\$M) & 4,117.4 && 4,323.27 && 4,539.43 && 4,766.4 && 5,004.73 && 5,254.96\\
PV cashflows (\$M) & 4,117.4 && 3,915.12 && 3,722.77 && 3,539.88 && 3,365.97 && 3,200.61\\
PV terminal value (\$M) &  && && && && && 40,667.48\\
\textbf{Total PV (\$M)} & 62,529.23\\
\textbf{Total PV / ICE supply (\$)} & 111.86\\
\textbf{ICE market price (\$)} & 94.04 \\
\midrule
\textbf{Nasdaq}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  1,376.0 && 1,444.8 && 1,517.04 && 1,592.89 && 1,672.54 && 1,756.16 \\
Workforce expenses (\$M) & 	412.8 && 433.44 && 455.11 && 477.87 && 501.76 && 526.85\\
Net income (\$M) & 963.2 && 1,011.36 && 1,061.93 && 1,115.02 && 1,170.78 && 1,229.31\\
PV cashflows (\$M) & 963.2 && 917.06 && 873.14 && 831.32 && 791.5 && 753.59\\
PV terminal value (\$M) &  && && && && && 9,720.70\\
\textbf{Total PV (\$M)} & 14,850.51\\
\textbf{Total PV / NDAQ supply (\$)} & 90.28\\
\textbf{NDAQ market price (\$)} & 152.54 \\
\midrule

\textbf{Chicago Board of Trade}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  870.2 && 913.71 && 959.4 && 1,007.36 && 1,057.73 && 1,110.62 \\
Workforce expenses (\$M) & 	261.06 && 274.11 && 287.82 && 302.21 && 317.32 && 333.19\\
Net income (\$M) & 609.14 && 639.6 && 671.58 && 705.16 && 740.41 && 777.43 \\
PV cashflows (\$M) & 609.14 && 578.98 && 550.32 && 523.07 && 497.17 && 472.56\\
PV terminal value (\$M) &  && && && && && 5,976.65\\
\textbf{Total PV (\$M)} & 9,207.89\\
\textbf{Total PV / CBOE supply (\$)} & 86.71\\
\textbf{CBOE market price (\$)} & 113.19 \\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 30\% respectively. 
\end{table*}

==> tables/dcf_crypto_historical.tex <==
\begin{table*}\centering

\caption{\acp{DAO}' historical balance sheets.}
\label{table:crypto_historical_data}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrrrrrrrr@{}}\toprule
& \multicolumn{1}{c}{$2020$} &  
\phantom{abc} & \multicolumn{4}{c}{$2021$} &
\phantom{abc} & \multicolumn{2}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{CQGR} \\
\cmidrule{2-2} \cmidrule{4-7}  \cmidrule{9-10}  \cmidrule{12-12}
& $Q4$ && $Q1$ & $Q2$ & $Q3$ & $Q4$ && $Q1$ & $Q2$ && \% \\ \midrule

\textbf{Uniswap}\\
Earnings (\$M) & $NA$ && 25.7 & 46.9 & 30.8 & 46.8 && 31.1 & 23.2 && \textit{-0.02\%}\\
\textit{\% growth} & \textit{$NA$} && \textit{$NA$} & \textit{82.33\%} & \textit{-34.33\%} & \textit{52.13\%} && \textit{-33.5\%} & \textit{-25.48\%} &&   \\

\textbf{Curve}\\
Earnings (\$M) & $NA$ && $NA$ & $NA$ & 6.34 & 19.8 && 18.5 & 12.2 && \textit{0.24\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{$NA$} & \textit{$NA$} & \textit{$NA$} & \textit{213.04\%} && \textit{-6.78\%} & \textit{-34.21\%} &&   \\

\textbf{Compound}\\
Earnings (\$M) & $NA$ && 10.6 & 10.9 & 9.0 & 10.0 && 4.8 & 1.8 && \textit{-0.30\%} \\
\textit{\% growth} & 	\textit{$NA$} && \textit{$NA$} & \textit{2.50\%} & \textit{-16.91\%} & \textit{11.14\%} && \textit{-51.89\%} & \textit{-62.69\%} &&  \\

\textbf{AAVE}\\
Earnings (\$M) & $NA$ && 1.2 & 5.5 & 9.3 & 12.7 && 6.5 & 6.0 && \textit{0.37\%} \\
\textit{\% growth} & 	\textit{$NA$} && \textit{$NA$} & \textit{355.22\%} & \textit{68.66\%} & \textit{35.94\%} && \textit{-48.84\%} & \textit{-8.08\%} &&  \\

\textbf{Yearn Finance}\\
Earnings (\$M) & $NA$ && $NA$ & 22.3 & 23.1 & 26.2 && 14.0 & 6.9 && \textit{-0.25\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{$NA$} & \textit{$NA$} & \textit{3.66\%} & \textit{12.98\%} && \textit{-46.55\%} & \textit{-50.29\%} &&   \\

\textbf{Idle Finance}\\
Earnings (\$M) & $NA$ && $NA$ & 0.3 & 0.2 & 0.2 && 0.1 & 0.05 && \textit{-0.37\%}\\
\textit{\% growth} & \textit{$NA$} && \textit{$NA$} & \textit{$NA$} & \textit{-36.96\%} & \textit{-24.12\%} && \textit{-59.15\%} & \textit{-20.77\%} &&   \\


\bottomrule
\end{tabular}
}
\end{table*}

==> tables/dcf_cyield_agg.tex <==
\begin{table*}
\centering
\caption{Asset management firms' \ac{NPV} evaluation using \ac{DCF}.}
\label{table:c_yield_valuation}
\ra{1.3}
\scalebox{0.60}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule

\textbf{Berkshire Hathaway}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  111,530.0 && 117,106.5 && 122,961.82 && 129,109.92 && 135,565.41 && 142,343.68 \\
Workforce expenses (\$M) & 	33,459.0 && 35,131.95 && 36,888.55 && 38,732.98 && 40,669.62 && 42,703.1 \\
Net income (\$M) & 78,071.0 && 81,974.55 && 86,073.28 && 90,376.94 && 94,895.79 && 99,640.58\\
PV cashflows (\$M) & 78,071.0 && 74,205.71 && 70,531.78 && 67,039.76 && 63,720.62 && 60,565.82\\
PV terminal value (\$M) &  && && && && && 765,995.62\\
\textbf{Total PV (\$M)} & 1,180,130.30\\
\textbf{Total PV / BRK.B supply (\$)} & 535.06\\
\textbf{BRK.B market price (\$)} & 273.02 \\
\midrule

\textbf{Morgan Stanley}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  15,814.0 && 16,604.7 && 17,434.94 && 18,306.68 && 19,222.02 && 20,183.12 \\
Workforce expenses (\$M) & 4,744.2 && 4,981.41 && 5,230.48 && 5,492.0 && 5,766.6 && 6,054.94\\
Net income (\$M) & 11,069.8 && 11,623.29 && 12,204.45 && 12,814.68 && 13,455.41 && 14,128.18\\
PV cashflows (\$M) & 11,069.8 && 10,644.02 && 10,234.61 && 9,840.96 && 9,462.44 && 9,098.48 \\
PV terminal value (\$M) &  && && && && && 132,466.85\\
\textbf{Total PV (\$M)} & 192,817.15\\
\textbf{Total PV / MS supply (\$)} & 111.91\\
\textbf{MS market price (\$)} & 76.10 \\
\midrule

\textbf{BlackRock}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  5,894.0 && 6,188.7 && 6,498.14 && 6,823.04 && 7,164.19 && 7,522.4  \\
Workforce expenses (\$M) & 	41,768.2 && 1,856.61 && 1,949.44 && 2,046.91 && 2,149.26 && 2,256.72\\
Net income (\$M) & 4,125.8 && 4,332.09 && 4,548.7 && 4,776.13 && 5,014.94 && 5,265.68 \\
PV cashflows (\$M) & 4,125.8 && 3,921.81 && 3,727.91 && 3,543.59 && 3,368.39 && 3,201.84\\
PV terminal value (\$M) &  && && && && && 40,528.04\\
\textbf{Total PV (\$M)} & 62,417.382\\
\textbf{Total PV / BLK supply (\$)} & 413.45\\
\textbf{BLK market price (\$)} & 609.04 \\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 30\% respectively. 
\end{table*}

==> tables/dcf_dex.tex <==
\begin{table*}\centering

\caption{\acp{DEX}' \ac{NPV} estimation using \ac{DCF}.}
\label{tab:dcf_dex}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule
\textbf{Uniswap}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  108.68 && 114.12 && 119.82 && 125.81 && 132.10 && 138.71\\
Workforce expenses (\$M) & 21.73 && 22.82 && 23.96 && 25.16 && 26.42 && 27.74\\
Net income (\$M) & 86.95 && 91.3 && 95.86 && 100.65 && 105.69 && 110.97\\
PV cashflows (\$M) & 86.95 && 73.04 && 61.35 && 51.54 && 43.29 && 36.36\\
PV terminal value (\$M) &  && && && && && 131.74\\
\textbf{Total PV (\$M)} & 484.26\\
\textbf{Total PV / UNI supply (\$)} & 1.06\\
\textbf{UNI market price (\$)} & 5.00 \\
\midrule
\textbf{Curve}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  61.31 && 64.37 && 67.59 && 70.97 && 74.52 && 78.25 \\
Workforce expenses (\$M) & 	12.26 && 12.87 && 13.51 && 14.19 && 14.90 && 15.65\\
Net income (\$M) & 49.05 && 51.5 && 54.08 && 56.78 && 59.62 && 62.6\\
PV cashflows (\$M) & 49.05 && 41.2 && 34.61 && 29.07 && 24.42 && 20.51\\
PV terminal value (\$M) &  && && && && && 74.31\\
\textbf{Total PV (\$M)} & 273.18\\
\textbf{Total PV / CRV supply (\$)} & 0.70\\
\textbf{CRV market price (\$)} & 0.69\\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 20\% respectively. 
\end{table*}

==> tables/dcf_plf.tex <==
\begin{table*}\centering

\caption{\acp{PLF}' \ac{NPV} estimation using \ac{DCF}.}
\label{table:dcf_plf}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule
\textbf{Compound}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  13.25 && 13.91 && 14.6 && 15.33 && 16.1 && 16.91 \\
Workforce expenses (\$M) & 	2.65 && 2.78 && 2.92 && 3.07 && 3.22 && 3.38\\
Net income (\$M) & 10.6 && 11.13 && 11.68 && 12.27 && 12.88 && 13.52\\
PV cashflows (\$M) & 10.6 && 8.9 && 7.48 && 6.28 && 5.28 && 4.43\\
PV terminal value (\$M) &  && && && && && 16.06\\
\textbf{Total PV (\$M)} & 59.02\\
\textbf{Total PV / COMP supply (\$)} & 8.59\\
\textbf{COMP market price (\$)} & 47.48 \\
\midrule
\textbf{AAVE}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  24.93 && 26.18 && 27.48 && 28.86 && 30.3 && 31.82 \\
Workforce expenses (\$M) & 	4.99 && 5.24 && 5.5 && 5.77 && 6.06 && 6.36\\
Net income (\$M) & 19.94 && 20.94 && 21.99 && 23.09 && 24.24 && 25.45\\
PV cashflows (\$M) & 19.94 && 16.75 && 14.07 && 11.82 && 9.93 && 8.34\\
PV terminal value (\$M) &  && && && && && 30.22\\
\textbf{Total PV (\$M)} & 111.07\\
\textbf{Total PV / AAVE supply (\$)} & 8.01\\
\textbf{AAVE market price (\$)} & 57.00 \\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 20\% respectively. 
\end{table*}

==> tables/dcf_stocks.tex <==
\begin{table*}\centering

\caption{Firms' historical earnings.}
\label{table:firms_historical_data}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrrrrrrrr@{}}\toprule
& \multicolumn{1}{c}{$2020$} &  
\phantom{abc} & \multicolumn{4}{c}{$2021$} &
\phantom{abc} & \multicolumn{2}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{CQGR} \\
\cmidrule{2-2} \cmidrule{4-7}  \cmidrule{9-10}  \cmidrule{12-12}
& $Q4$ && $Q1$ & $Q2$ & $Q3$ & $Q4$ && $Q1$ & $Q2$ && \% \\ \midrule

\textbf{ICE}\\
Earnings (\$M) & 583.0 && 674.0 & 833.0 & 1932.0 & 824.0 && 2109.0 & 832.0 && \textit{6.11\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{15.61\%} & \textit{23.59\%} & \textit{131.93\%} & \textit{-57.35\%} && \textit{155.95\%} & \textit{-60.55\%} && \\

\textbf{NDAQ}\\
Earnings (\$M) & 356.0 && 267.0 & 395.0 & 454.0 & 371.0 && 314.0 & 374.0 && \textit{0.83\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{-25.0\%} & \textit{47.94\%} & \textit{14.94\%} & \textit{-18.28\%} && \textit{-15.36\%} & \textit{19.11\%} &&  \\

\textbf{CBOE}\\
Earnings (\$M) & 163.4 && 122.9 & 192.9 & 179.2 & 173.8 && 210.2 & 224.9 && \textit{5.47\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{-24.79\%} & \textit{56.96\%} & \textit{-7.1\%} & \textit{-3.01\%} && \textit{20.94\%} & \textit{6.99\%} &&   \\

\textbf{C} \\
Earnings (\$M) & 5,441.0 && 10,309.0 & 7,348.0 & 5,862.0 & 3,950.0 && 5,266.0 & 5,971.0 && \textit{6.07\%} \\
\textit{\% growth} & \textit{37.61\%} && \textit{89.47\%} & \textit{-28.72\%} & \textit{-20.22\%} & \textit{-32.62\%} && \textit{33.32\%} & \textit{13.39\%} &&      \\


\textbf{BAC}\\
Earnings (\$M) & 4,546.0 && 6,119.0 & 9,166.0 & 8,042.0 & 8,950.0 && 7,818.0 & 7,879.0 && \textit{9.6\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{34.6\%} & \textit{49.8\%} & \textit{-12.26\%} & \textit{11.29\%} && \textit{-12.65\%} & \textit{0.78\%} &&    \\

\textbf{WFC}\\
Earnings (\$M) & 3,866.0 && 5,591.0 & 8,189.0 & 6,926.0 & 8,110.0 && 4,509.0 & 3,565.0 && \textit{1.03\%} \\
\textit{\% growth} & \textit{16.52\%} && \textit{44.62\%} & \textit{46.47\%} & \textit{-15.42\%} & \textit{17.1\%} && \textit{-44.4\%} & \textit{-20.94\%} &&     \\

\textbf{BRK.B} \\
Earnings (\$M) & 37,930.0 && 45,403.0 & 14,528.0 & 35,721.0 & 12,484.0 && 48,953.0 & 6,812.0 && \textit{-24.89\%} \\
\textit{\% growth} & \textit{$NA$} && \textit{19.7\%} & \textit{-68.0\%} & \textit{145.88\%} & \textit{-65.05\%} && \textit{292.13\%} & \textit{-86.08\%} &&       \\

\textbf{MS} \\
Earnings (\$M) & 4,430.0 && 5,344.0 & 4,566.0 & 4,874.0 & 4,884.0 && 4,588.0 & 3,319.0 && \textit{-0.7\%} \\
\textit{\% growth} & \textit{27.04\%} && \textit{20.63\%} & \textit{-14.56\%} & \textit{6.75\%} & \textit{0.21\%} && \textit{-6.06\%} & \textit{-27.66\%} &&       \\

\textbf{BLK} \\
Earnings (\$M) & 2,167.0 && 1,591.0 & 2,201.0 & 2,271.0 & 2,110.0 && 1,626.0 & 1,321.0 && \textit{-5.62\%} \\
\textit{\% growth} & \textit{9.39\%} && \textit{-26.58\%} & \textit{38.34\%} & \textit{3.18\%} & \textit{-7.09\%} && \textit{-22.94\%} & \textit{-18.76\%} &&       \\




\bottomrule
\end{tabular}
}
\end{table*}

==> tables/dcf_yearn_agg.tex <==
\begin{table*}\centering

\caption{Yield aggregators' \ac{NPV} evaluation using \ac{DCF}.}
\label{tab:dcf_yearn}
\ra{1.3}
\scalebox{0.6}{
\begin{tabular}{@{}rrrrrrcrrrrrr@{}}\toprule
&  \multicolumn{1}{c}{$2022$} &
\phantom{abc} & \multicolumn{1}{c}{$2023$} &
\phantom{abc} & \multicolumn{1}{c}{$2024$} &
\phantom{abc} & \multicolumn{1}{c}{$2025$} &
\phantom{abc} & \multicolumn{1}{c}{$2026$} &
\phantom{abc} & \multicolumn{1}{c}{$2027$}\\ \midrule

\textbf{Yearn Finance}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  41.87 && 43.96 && 46.16 && 48.47 && 50.9 && 53.44 \\
Workforce expenses (\$M) & 	8.37 && 8.79 && 9.23 && 9.69 && 10.18 && 10.69\\
Net income (\$M) & 33.5 && 35.17 && 36.93 && 38.78 && 40.72 && 42.75\\
PV cashflows (\$M) & 33.5 && 28.14 && 23.64 && 19.85 && 16.68 && 14.01\\
PV terminal value (\$M) &  && && && && && 50.75\\
\textbf{Total PV (\$M)} & 	186.56\\
\textbf{Total PV / YFI supply (\$)} & 5,902.42\\
\textbf{YFI market price (\$)} & 5,419.10 \\
\midrule
\textbf{Idle Finance}\\
% \% growth rate &  $NA$  && 5 && 5 && 5 && 5 && 5\\
Revenue (\$M)  &  0.25 && 0.26 && 0.27 && 0.28 && 0.3 && 0.31 \\
Workforce expenses (\$M) & 	0.05 && 0.05 && 0.05 && 0.06 && 0.06 && 0.06\\
Net income (\$M) & 0.2 && 0.21 && 0.22 && 0.23 && 0.24 && 0.25\\
PV cashflows (\$M) & 0.2 && 0.16 && 0.14 && 0.12 && 0.1 && 0.08\\
PV terminal value (\$M) &  && && && && && 0.30\\
\textbf{Total PV (\$M)} & 1.10\\
\textbf{Total PV / IDLE supply (\$)} & 0.41\\
\textbf{IDLE market price (\$)} & 0.23 \\
\bottomrule
\end{tabular}
}
\newline\scriptsize
Note: market prices are retrieved on 30 June 2022. 
The annual growth rate for revenue and workforce expenses equals 5\% and 20\% respectively. 
\end{table*}
